Learning Stable Deep Dynamics Models

Deep networks are commonly used to model dynamical systems, predicting how the state of a system will evolve over time (either autonomously or in response to control inputs). Despite the predictive power of these systems, it has been difficult to make formal claims about the basic properties of the learned systems. In this paper, we propose an approach for learning dynamical systems that are guaranteed to be stable over the entire state space. The approach works by jointly learning a dynamics model and Lyapunov function that guarantees non-expansiveness of the dynamics under the learned Lyapunov function. We show that such learning systems are able to model simple dynamical systems and can be combined with additional deep generative models to learn complex dynamics, such as video textures, in a fully end-to-end fashion.

==> figures/pendulum_results/8.tex <==
\pgfplotstableread{figures/pendulum_results/8_simple.dat}{\pendressimple}
\pgfplotstableread{figures/pendulum_results/8_REHU_0.005.dat}{\pendressrehu}

\begin{figure}
    \begin{tikzpicture}[scale=1]
    \begin{axis}[
        axis on top,% ----
        scale only axis,
        enlargelimits=false,
        xmin=0, ymin=0, 
    xmax=1000,
        width=5.0in,
        height=1.404in,
        ylabel near ticks,
        legend pos=north west]


    \end{axis}
    \end{tikzpicture}
\caption{Error in predicting $
\theta, \dot \theta$ in 8-link pendulum over time.}
    \label{fig:link_8_results}
\end{figure}


==> figures/pendulum_results/nlinks.tex <==
\pgfplotstableread{figures/pendulum_results/nlinkerror_simple.dat}{\nlinkerrorsimple}
\pgfplotstableread{figures/pendulum_results/nlinkerror_rehu.dat}{\nlinkerrorrehu}

\begin{figure}
    \begin{tikzpicture}[scale=1]
    \begin{axis}[
        axis on top,% ----
        scale only axis,
        enlargelimits=false,
        xmin=.5, ymin=0, xmax=8.5,
        width=5.0in,
        height=1.404in,
        xlabel={Number of links in pendulum},
        ylabel={Error at 1000 timesteps},
        ylabel near ticks,
        legend pos=north west,
        xtick=data]

    \addplot+[y filter/.code={\pgfmathparse{#1/500}\pgfmathresult}]
        table [x={n}, y={loss}] {\nlinkerrorsimple};
    \addplot+[y filter/.code={\pgfmathparse{#1/500}\pgfmathresult}]
        table [x={n}, y={loss}] {\nlinkerrorrehu};
    \legend{Simple Model,Stable Model}
    \end{axis}
    \end{tikzpicture}
\caption{Error in predicting $
\theta, \dot \theta$ as the number of links in the pendulum increases.}
    \label{fig:nlink_results}
\end{figure}


==> figures/tricks.tex <==

% Display graphics in pgfplots without deformation: https://tex.stackexchange.com/a/338627
\makeatletter
\newcommand\addplotgraphicsnatural[2][]{%
    \begingroup
    % set options in this local group (will be lost afterwards):
    \pgfqkeys{/pgfplots/plot graphics}{#1}%
    % measure the natural size of the graphics:
    \setbox0=\hbox{\includegraphics{#2}}%
    %
    % compute the required unit vector ratio:
    \pgfmathsetmacro{\xfactor}{\wd0/(\pgfkeysvalueof{/pgfplots/plot graphics/xmax} - \pgfkeysvalueof{/pgfplots/plot graphics/xmin})}%
    \pgfmathsetmacro{\yfactor}{\ht0/(\pgfkeysvalueof{/pgfplots/plot graphics/ymax} - \pgfkeysvalueof{/pgfplots/plot graphics/ymin})}\yfactor%
    % The smaller of the unit vectors should be 1, so the other needs to be scaled appropriately
    \pgfmathsetmacro{\xunit}{\xfactor<\yfactor ? 1 : \xfactor/\yfactor}
    \pgfmathsetmacro{\yunit}{\xfactor<\yfactor ? \yfactor/\xfactor : 1}
    %
    % configure pgfplots to use it.
    % The \xdef expands all macros except those prefixed by '\noexpand'
    % and assigns the result to a global macro named '\marshal'.
    \xdef\marshal{%
        \noexpand\pgfplotsset{unit vector ratio*={\xunit\space \yunit}}%
    }%
    \endgroup
    %
    % use our macro here:
    \marshal
    %
    \addplot graphics[#1] {#2};
}   
\makeatother
